Extending Partial Representations of Subclasses of Chordal Graphs

Chordal graphs are intersection graphs of subtrees of a tree T. We investigate the complexity of the partial representation extension problem for chordal graphs. A partial representation specifies a tree T' and some pre-drawn subtrees of T'. It asks whether it is possible to construct a representation inside a modified tree T which extends the partial representation (i.e, keeps the pre-drawn subtrees unchanged). We consider four modifications of T' and get vastly different problems. In some cases, it is interesting to consider the complexity even if just T' is given and no subtree is pre-drawn. Also, we consider three well-known subclasses of chordal graphs: Proper interval graphs, interval graphs and path graphs. We give an almost complete complexity characterization. We further study the parametrized complexity of the problems when parametrized by the number of pre-drawn subtrees, the number of components and the size of the tree T'. We describe an interesting relation with integer partition problems. The problem Partition is used for all NP-completeness reductions. The extension of interval graphs when the space in T' is limited is "equivalent" to the BinPacking problem.

==> Makefile <==
extending_chor_journal:
	cat extending_chor_journal.aux | sed -n '/\\bib/p' > mpost.aux
	mpost extending_chor_journal.mp
	latex extending_chor_journal.tex
	dvips extending_chor_journal.dvi
	ps2pdf extending_chor_journal.ps
	pspdftool "bbox scaleto(a4)" extending_chor_journal.pdf extending_chor_journal_print.pdf

bibtex:
	latex extending_chor_journal.tex
	bibtex extending_chor_journal
	latex extending_chor_journal.tex
	latex extending_chor_journal.tex

gzip:
	-rm extending_chor_journal.tar.gz
	tar cvzf extending_chor_journal.tar.gz *
	
zip:
	-rm extending_chor_journal.zip
	zip extending_chor_journal.zip *.tex *.eps *.mp *.pdf *.ps *.bib *.sty *.bst

